Future Scenarios and Challenges for Security and Privacy

Over the past half-century, technology has evolved beyond our wildest dreams. However, while the benefits of technological growth are undeniable, the nascent Internet did not anticipate the online threats we routinely encounter and the harms which can result. As our world becomes increasingly connected, it is critical we consider what implications current and future technologies have for security and privacy. We approach this challenge by surveying 30 predictions across industry, academia and international organisations to extract a number of common themes. Through this, we distill 10 emerging scenarios and reflect on the impact these might have on a range of stakeholders. Considering gaps in best practice and requirements for further research, we explore how security and privacy might evolve over the next decade. We find that existing guidelines both fail to consider the relationships between stakeholders and do not address the novel risks from wearable devices and insider threats. Our approach rigorously analyses emerging scenarios and suggests future improvements, of crucial importance as we look to pre-empt new technological threats.

==> old_section_three.tex <==

\section{Challenges for Security and Privacy}
\label{sec:four} 

As a next stage, we reflect on the future applicability of existing `best practice' guidelines for \textbf{individuals}, \textbf{organisations} and \textbf{nations}. This is of great importance, as these documents inform stakeholder groups and would be expected to guard against emerging threats. We summarise the gaps in current frameworks, focusing on several key examples due to space restrictions, and point to required research and development. At the individual level, we consider the main UK and US government initiatives for improving individuals' cybersecurity practices: for the UK, the Cyber Streetwise campaign \cite{cyberstreetwise}, and for the US, Stop.Think.Connect \cite{stopthinkconnect}. The UK Get Safe Online initiative was also considered, but this is private sector and less authoritative than Cyber Streetwise. For organisations, we examine the US National Institute for Standards and Technology's (NIST) cybersecurity framework \cite{NIST}, and the Center for Internet Security's Critical Security Controls (CIS CSC) \cite{sans}, which provide key corporate guidelines. The International Telecommunication Union National Cybersecurity Strategy Guide \cite{ITU} and NATO National Cybersecurity Framework Manual \cite{NATO} are considered as internationally-recognised guidelines for nations. Based on our findings, we conclude this section with a call to action for researchers, stakeholders and policy makers.

\subsection{Gaps in existing guidelines}

While advantageous for the present day, \textbf{awareness campaigns for individuals} do not translate to a future in which the IoT pervades daily life. In this future, individuals' understanding of, and agency over, their online presence is key to the protection of their privacy. Current campaigns go some way to promoting good practice in this area (e.g. recommendations for protecting privacy when using social media \cite{cyberstreetwise}; privacy-protecting recommendations given for the use of web services, devices, purchase history, and location \cite{stopthinkconnect}). However, these initiatives do not extend to educating citizens on the privacy implications of increasingly-used wearable, biometric and sensor-based technologies. Nor is clear usable advice given on the specific types of data collected by different applications and devices. For guidelines to be suitable for future scenarios, awareness campaigns must focus on emerging technologies and give specific, practical advice for maintaining security and privacy in a world focused on big data. Furthermore, these public initiatives should be periodically evaluated to ascertain their effectiveness in improving individuals' behaviour. Whether undertaken through large-scale surveys or targeted focus groups, feedback mechanisms would allow for campaigns to be iteratively refined over time. 

\textbf{Existing frameworks for organisations} do not adequately address those human aspects which will be key to future corporate cybersecurity. The NIST and CSC documents \cite{NIST, sans} are highly comprehensive, with useful references to external guidelines. They do not, however, provide frameworks within which the increasingly-important human aspects of organisational cybersecurity can be addressed; namely, problems arising from insider threats and BYOD. For instance, NIST aims to mitigate insider threats by recommending the comparison of personnel actions against expected behaviours and data-flow baselines. CSC addresses the problem by advocating controlled use of administrative priveleges, access controls set on a ``need to know" basis, and monitoring and control of employee and contractor accounts. While these activities are essential, tracking employee activity alone will not always be adequate to defend against insiders who may themselves be aware of the monitoring systems in place \cite{colwill2009human}. Unfortunately, both frameworks fail to give any consideration to the growing need to study the motives of personnel or to monitor behaviour from a psychological perspective.

Both the NIST and CSC recommendations protect organisations against risks from BYOD policies insofar as it is specified that physical devices and systems should be inventoried and monitored. We foresee a huge expansion in the ownership of IoT devices, which will result in an increase in the number of personally-owned devices present in the workplace; in particular, wearables and implants. In this future, far from remote with the increased popularity of smart watches and fitness monitors, cataloguing all connected products will not be feasible. More sophisticated means of mitigating IoT and BYOD risk are required \cite{Nurse2015}, such as network protection against potentially-invisible devices (e.g. implanted medical chips) without requiring strict inventory. This is crucial to recognising the increasing blur between internal and external spaces.

\textbf{Cybersecurity frameworks for nations} \cite{NIST, sans} recommend international cooperation to unite national strategies. Set against our future scenarios, this is extremely optimistic, especially between non-allied states. Indeed, it is predicted that heterogeneous state postures and differing cybersecurity laws will stifle international cooperation. This combined with the proliferation of cyber weaponry and problems of attribution suggests that the unification of national strategies is unrealistic. Of greater importance is the construction of policies and legislation which allows states to suit their own, and international, interests in a non-unified cyber landscape.

Based on our scenarios, we foresee that both state-level cyber weaponry will grow and international tensions will escalate as a result of high-profile cyber incidents. A recent example of expected events is the unattributed Ukrainian power outage of December 2015, apparently caused by a cyber-attack \cite{BBCNews2016}. Currently, agreement of those terms key to building legislation for international incidents is lacking. For example, there are no widely-agreed definitions for either ``cyber warfare'' or ``cyber attack'' \cite{NATO}. Legislation in this area is crucial to maintaining order in the coming decades. 

\subsection{Requirements for research and development}

Based on the gaps identified, much work is required to extend cybersecurity frameworks for the future. We detail areas that must be addressed through academic research, the development of policy, and action by stakeholders.

\textbf{For the protection of individuals'} privacy in a data-rich world, policies and laws on collection, storage and processing must be reconsidered in light of the increased sensitivity and abundance of data. Education will be central to affording citizens the understanding to retain agency over their information, with progress monitored through national cybersecurity surveys. Usable solutions for privacy protection should also be developed, such as applications which highlight the data collected by wearable devices.

\textbf{For organisations}, research into the human aspects of insider threat, such as behavioural psychology and potential motives, is important. Both the corporate adoption of education schemes and the consideration of employees' actions are critical to proactively detecting insider threats. Whilst existing studies have began to explore the psychological, behavioural, cultural and technical characteristics of insider threats \cite{Nurse2014}, further research is required to develop comprehensive solutions that are ultimately useful for organisations. The evolution of current practice is crucial if companies wish to maintain resistance against increasingly-sophisticated insider threats. 

BYOD currently poses a number of organisational challenges \cite{Nurse2015,garba2015review} and our emerging scenarios suggest this situation will only be exacerbated. To protect companies against the increased number and variety of personal devices brought to the office, two requirements are crucial. Firstly, applications should be developed to secure company networks against the risks posed by personal technologies. Secondly, effective organisational policies must be implemented to manage risk in a future pervaded by wearable and implanted devices.

\textbf{At the national level}, more specificity is required in calls for international cooperation. Whilst some states will negotiate mutual agreements on offensive cyber actions, as the US and China did in their 2015 Cyber Agreement \cite{Rosenfeld2015}, the global unification of security postures is highly unlikely. As such, both international cybersecurity bodies and frameworks for addressing key matters, such as piracy and cross-border law enforcement, must function in a heterogeneous environment. As offensive cyber weapons proliferate and global tensions increase, legislation on `acts of war' and digitally-proportionate responses must be defined. It is inevitable that nation-state cyber weaponry will reach the black market, and it is crucial that the consequences of its use are understood, and controls placed around it, to avoid heightening of risks in the most harmful of circumstances \cite{hodgescreese}. 

\textbf{Interactions between individuals, organisations and nations} must also be considered. We have explored the future scenario impact on our three stakeholders separately. In reality, there are several relationships and dependencies between them. For example, the effect that advances in machine learning will have on individuals' privacy will depend largely on both the regulations governing data collection and the behaviour of organisations. There is, however, no single document that details cybersecurity guidelines across these three different levels. This lack of cohesion introduces complex subtleties and key dependencies can be missed. Broad frameworks would enable a clear vision of both current cybersecurity practices and their future weaknesses, though it would be challenging to locate a party capable of constructing such a comprehensive document. This is especially true considering the international nature of the field, with recommendations required to be equally applicable in a Chinese power station and a US bank. Specificity is by definition in tension with generality, and new guidelines would also require frequent update to ensure they are suitable.


==> old_section_two.tex <==
\section{Emerging Technology Futures}
\label{sec:two}

We begin by surveying existing predictions before consolidating key commonalities into our representative emerging scenarios.

\subsection{Surveyed predictions}

Schwartz \cite{Schwartz2011}, writing under the Center for a New American Security, considered both optimistic and pessimistic scenarios. Through his analyses of policy and technology, he identified several possibilities, in addition to indicators to judge cybersecurity progress. His considerations included the construction of multiple national internets and the ubiquity of online threats due to the proliferation of cheap attack tools.

Hunter \cite{Hunter2013}, performing organisational research through Gartner, plotted an x-axis from individual to enterprise targets against a y-axis from tribal to monolithic authority. His scenario quadrants were denoted as: regulated risk (the establishment of software liability), coalition rule (the growth of underground hackers), controlling parent (the development of surveillance societies), and neighbourhood watch (the construction of segregated networks).

The World Economic Forum \cite{WorldEconomicForum2014} collated knowledge from interviews and workshops with global executives. Through this, they considered expert feedback before constructing scenarios and presenting a 14-point roadmap for collaboration. The findings were drawn into three future possibilities: hackers retaining an advantage and stunting economic growth, frequent attacks deterring citizens from online services, or strong resilience triggering further technological innovation.

The International Cyber Security Protection Alliance \cite{InternationalCyberSecurityProtectionAlliance2013} theorised several future scenarios through their Project 2020 initiative. Through collaboration with the Trend Micro security firm, ICSPA analysed the current threat landscape and validated their concepts by an expert panel. Three narratives were discussed: a second-generation digital native, a business in a highly-technological market, and a nation state capitalising from security expertise.

Burt \textit{et al.} \cite{Burt2014} developed the Microsoft Cyberspace2025 report, considering scenarios grounded in a econometric model. In addition to the quantitative analysis of 100 socioeconomic indicators over 80 nation states, qualitative insights were sourced from researchers and experts. They constructed three future scenarios: `peak' comprising the global embracement of technology, `plateau' representing piecemeal cyber adoption, and `canyon' theorising protectionist security strategies.

The Berkeley Center for Long-Term Cybersecurity \cite{BerkeleyCenterforLong-TermCybersecurity2015} convened an interdisciplinary conference with expertise from computer science and politics. From nascent ideas formed during the sessions, Berkeley graduate researchers developed the concepts into five detailed narratives. These comprised the Internet becoming an anarchy, radical advances in machine learning, the technology bubble bursting, Internet of Things surveillance, and the monitoring of human emotions. 

In a 2015 article, Benzel \cite{Benzel2015} described discussions from a recent US DHS session concerning cybersecurity research and development. The event saw a number of working groups deliberating those objectives which should be prioritised over the next five years. The resulting recommendations included increasing the role of the private sector and developing metrics to evaluate cybersecurity return on investment (ROI).

In academic work, Choo \cite{Choo2011} conducted an exploration of cybercrime and how this might evolve in the future. Through considering affairs in the US, UK and Australia, he constructed several predictions and suggested criminological prevention strategies. The scenarios ranged from the use of social media portals for propaganda purposes to the escalation of international tensions through frequent cyber-attacks.

\subsection{Representative scenarios}

After surveying the range of future possibilities from academia, industry and international organisations, we extracted their key commonalities. This was performed through several iterations of manual coding until we identified a shortlist of recurring concepts. These were then constructed into 10 representative emerging scenarios considering the technological, political and commercial possibilities of the following two decades.

These are as follows:
\begin{enumerate}
  \item The Internet of Things pervades daily life, blurring the physical and virtual worlds. This entanglement leads to online risks becoming increasingly intangible, contributing to further cyber-threats.
  \item The proliferation of simple attack tools and government investments in offensive capabilities contributes to frequent high-profile cyber incidents. Nation-state weaponry leaks onto the black market and is reused by cybercriminals to steal customer data from organisations.
  \item Whilst many states take liberal risk-based approaches, several favour repressive means to enforce order online. This leads to the censorship and surveillance of their populations, damaging cross-border trade and placing democracy under pressure.
  \item The heterogeneity of state technology postures stifles international agreement and cooperation over cyber norms. This increases global tensions as attacks increasingly come from safe havens who refuse to prosecute their cyber criminals. 
  \item The concept of intellectual property evolves as traditional business models are placed under increasing pressure from both pirates and new competitors. Traditional market leaders fall and sell their data assets to innovative firms better-equipped to operate in challenging environments.
  \item Big data and machine learning supports prediction and manipulation of individuals by corporations, marketers and governments. Sophisticated statistical analysis enables companies to tailor their advertisements on an unprecedented scale, whilst political parties customise their releases to target individual citizens.
  \item Private organisations continue to know more about their customers than national governments, leading to the growth of public-private data-sharing partnerships. Whilst these arrangements are deemed beneficial to national security, large parts of critical infrastructure remain owned by multinational corporations.
  \item The concept of privacy is reinterpreted by ``digital natives'' who have been raised in an age of social networking and ubiquitous Internet access. Individuals become accustomed to the development of invasive technologies which offer great benefits to convenience and productivity.
\end{enumerate}

\subsection{Asset impact}

We then proceeded to consider our representative emerging scenarios and the impact they could have on a number of critical assets: \textit{data}, \textit{information}, \textit{PII (Personally Identifiable Information)}, \textit{intelligence} and \textit{organisations}.

The pervasion of the Internet of Things would have many implications for data, including a greater scale of aggregation, the collection of physical data and opportunities for covert surveillance. Information, both geographical and topological, could be applied in more locations, whilst edge intelligence would enable sophisticated communications. The IoT would allow PII to be captured with greater ease and potentially enable the monitoring of sensitive biometric data. Intelligence could be enhanced through covert device surveillance, geographic tracking of nodes and eavesdropping on remote conversations.  Organisations could experience the benefits from shipment monitoring and tool automation, but must protect their networks from an increased number of potentially-hostile devices.

The proliferation of attack tools would place data under increased risk, by expanding both the capability and range of actors who could infiltrate a network. The integrity of information would be placed under greater suspicion, with the costs of protecting records increasing correspondingly. Attack tools could either contribute to a constant risk of identity theft or actually nullify the importance of leaked PII. Whilst investment in offensive technologies creates further opportunities for intelligence collection, the democratisation of such weapons could place agencies at risk of counterespionage. Organisations might have a reduced willingness to store data remotely, making use of cyber-insurance to mitigate their risk exposure.

The repressive enforcement of online order would imply widespread censorship, filtering and data sharing restrictions. These approaches could contribute to a growth in government propaganda, certain information being considered seditious and the deletion of undesirable records. In such regimes, PII could be used to identify and target citizens, with the enforcement of identity documents connecting online and offline personae. Intelligence gathering would be greatly enhanced in these states, with the compilation of citizen dossiers. However, business would be stifled through online restrictions, increased regulation and protectionist levies placed on technology.

The heterogeneity from state postures will offer little cross-border data protection, reduce collaborative data sharing and encourage rival nations to continue offensive operations. This would contribute to increased risks from foreign espionage, raising the costs of protecting sensitive information. Differing definitions of PII across states would obstruct consensus and remove the accountability of repressive regimes. Heterogeneous technology postures would reduce intelligence sharing, potentially increasing global threats, and heightening incentives to exfiltrate foreign data. Differing approaches would damage organisations, with challenges expanding into new regions and unpredictable international relations contributing to market instability.

The evolution of new business models will see data as an important commodity, increasingly traded in data exchanges and sold by organisations which go bankrupt. Whilst information will become the most valuable corporate asset, it will continue to be vulnerable to copyright infringement. PII aggregations will be traded by corporations due to their value for predicting and profiling consumers. The new data-rich companies dominating the markets present novel opportunities for intelligence gathering, whether covertly or through public-private partnerships. Competition will expand as start-ups vie with established vendors, and sales of physical products will be rapidly replaced by virtual goods.

Advances in big data and machine learning will result in data being processed and collected in unprecedented volumes, with these metrics supporting intelligent decision-making. Information could be efficiently generated through machine learning algorithms, with increasingly-large digital dossiers held on consumers. PII could be inferred through novel techniques, correlated with other metrics or used to profile individuals and their spending habits. Intelligence could be generated or corroborated through sophisticated forecasting, or used as a means of conditioning and manipulating targets. In the commercial world, data becomes the most valuable commodity, with improved targeted advertising and financial predictions delivering increased revenues.

Public-private data-sharing partnerships lead to corporate records being exchanged for government threat intelligence. PII could assist the tracking or surveillance of citizens, but the duplication of this data increases the chance that sensitive details will be leaked. Governments can enhance their intelligence by corroborating information from multiple organisations, though sharing data with private companies might require non-disclosure agreements. Whilst partnerships might increase situational awareness, PR might be damaged by this arrangement and foreign consumers be deterred from disclosing their data.

Reinterpretations of privacy could lead to data being voluntary disclosed in greater quantities, in addition to the increased use of online services and the growing reputational importance of data integrity. Information will be shared on an unprecedented scale, with instant access considered standard and online repositories swelling in size. PII could lose its sensitivity as more-personal details, such as sexual orientation or political affiliation, proliferate the web. Whilst open source intelligence will be available in increased quantities, there is greater risk of confidential records being leaked. Corporations will benefit from public data and social media analytics, with individuals increasingly willing to exchange personal details for convenience.

==> section_three_old.tex <==

\section{Challenges for Security and Privacy}
\label{sec:four} 

We reflect on the future applicability of existing `good practice' guidelines for \textbf{individuals}, \textbf{organisations} and \textbf{nations}. We summarise the gaps in current frameworks, focusing on several key examples due to space restrictions, and point to required research and development. At the individual level, we consider the main UK and US government initiatives for improving individuals' cybersecurity practices: for the UK, the Cyber Streetwise campaign \cite{cyberstreetwise}, and for the US, Stop.Think.Connect \cite{stopthinkconnect}. For organisations, we examine the US National Institute for Standards and Technology's (NIST) cybersecurity framework \cite{NIST}, which provides key corporate guidelines. The International Telecommunication Union National Cybersecurity Strategy Guide \cite{ITU} and NATO National Cybersecurity Framework Manual \cite{NATO} are considered as internationally-recognised guidelines for nations. Based on our findings, we conclude this section with a call to action for researchers, stakeholders and policy makers.

\subsection{Gaps in existing guidelines}

For \textbf{individuals}, the awareness campaigns considered do not translate to a future in which the IoT pervades daily life and and new types of sensitive data, including bio-data, are widely available. In this future, individuals' understanding of, and agency over, their online presence is key to the protection of their privacy. Current campaigns go some way to promoting good practice in this area (recommendations for protecting privacy when using social media \cite{cyberstreetwise}; privacy-protecting recommendations given for the use of web services, devices, purchase history, and location \cite{stopthinkconnect}). However, these initiatives do not extend to educating citizens on the privacy implications of increasingly-used wearable, biometric and sensor-based technologies. Nor is clear usable advice given on the specific types of data collected by different applications and devices. For guidelines to be suitable for future scenarios, awareness campaigns must focus on emerging technologies and give specific, practical advice for maintaining privacy in a world of big data.

Existing frameworks for \textbf{organisations} do not adequately address those human aspects which will be key to future corporate cybersecurity. The NIST document \cite{NIST} is highly comprehensive, with useful references to external guidelines. It does not, however, provide a framework within which the increasingly-important human aspects of organisational cybersecurity can be addressed; namely, problems arising from insider threats and BYOD. NIST aims to mitigate organisational insider threat by recommending the comparison of personnel actions against expected behaviours and data-flow baselines. While this is essential, tracking employee activity alone will not always be adequate to defend against insiders who may themselves be aware of the monitoring systems in place \cite{colwill2009human}. Unfortunately, the framework fails to give any consideration to the growing need to study the motives of personnel or to monitor behaviour from a psychological perspective.

The NIST recommendations in protect organisations against risks from BYOD policies insofar as it is specified that physical devices and systems should be inventoried. We foresee a huge expansion in the ownership of IoT devices, which will result in an increase in the number of personally-owned devices present in the workplace; in particular, wearables and implants. In this future, far from remote with the increased popularity of smart watches and fitness monitors, cataloguing all connected products will not be feasible. More sophisticated means of mitigating BYOD risk are required \cite{Nurse2015}, such as network protection against potentially-invisible devices (e.g. implanted medical chips) without requiring strict inventory.

For \textbf{nations}, cybersecurity frameworks recommend international cooperation to unite national strategies. Set against our future scenarios, this is extremely optimistic, especially between non-allied states. Indeed, it is predicted that heterogeneous state postures and differing cybersecurity laws will stifle international cooperation. This combined with the proliferation of cyber weaponry and problems of attribution suggests that the unification of national strategies is unrealistic. Of greater importance is the construction of policies and legislation which allows states to suit their own, and international, interests in a non-unified cyber landscape.

Based on our scenarios, we foresee that both state-level cyber weaponry will grow and international tensions will escalate as a result of high-profile cyber incidents. A recent example of expected events is the unattributed Ukrainian power outage of December 2015, apparently caused by a cyber-attack \cite{BBCNews2016}. Currently, agreement of those terms key to building legislation for international incidents is lacking. For example, there are no widely-agreed definitions for either ``cyber warfare'' or ``cyber attack'' \cite{NATO}. Legislation in this area is crucial to maintaining order in the coming decades. 

\subsection{Requirements for research and development}

Based on the gaps identified, much work is required to extend cybersecurity frameworks for the future. For the protection of \textbf{individuals'} privacy in a data-rich world, policies and laws on collection, storage and processing must be reconsidered in light of the increased sensitivity and abundance of data. Education will be central to affording citizens the understanding to retain agency over their information, with progress monitored through national cybersecurity surveys. Usable solutions for privacy protection should also be developed, such as applications which highlight the data collected by wearable devices.

For \textbf{organisations}, research into the human aspects of insider threat, such as behavioural psychology and potential motives, is important. Both the corporate adoption of education schemes and the consideration of employees' actions are critical to proactively detecting insider threats. Whilst existing studies outline some work needed in this area \cite{colwill2009human}, further research is required to develop solutions that are useful for organisations. The evolution of current practice is crucial if companies wish to maintain resistance against increasing-sophisticated insider threats. 

BYOD currently poses a number of organisational challenges \cite{garba2015review} and our emerging scenarios suggest this situation will only be exacerbated. To protect companies against the increased number and variety of personal devices brought to the office, two requirements are crucial. Firstly, applications should be developed to secure company networks against the risks posed by personal technologies. Secondly, effective organisational policies must be implemented to manage risk in a future pervaded by wearable and implanted devices.

At the \textbf{national} level, more specificity is required in calls for international cooperation. Whilst some states will negotiate mutual agreements on offensive cyber actions, as the US and China did in their 2015 Cyber Agreement \cite{Rosenfeld2015}, the global unification of security postures is highly unlikely. As such, both international cybersecurity bodies and frameworks for addressing key matters, such as piracy and cross-border law enforcement, must function in a heterogeneous environment. As offensive cyber weapons proliferate and global tensions increase, legislation on acts of war and digitally-proportionate responses must be defined.

We have considered the future scenario impact on our three stakeholders separately. In reality, there are several relationships and dependencies between individuals, organisations and nations. For example, the effect that advances in machine learning will have on individuals' privacy will depend largely on both the regulations governing data collection and the behaviour of organisations. There is, however, no single document that details cybersecurity guidelines across these three different levels. This lack of cohesion introduces complex subtleties and key dependencies can be missed. Broad frameworks would enable a clear vision of both current cybersecurity practices and their weaknesses when projected into the future.

